Detecting hidden confounding in observational data using multiple environments

A common assumption in causal inference from observational data is that there is no hidden confounding. Yet it is, in general, impossible to verify this assumption from a single dataset. Under the assumption of independent causal mechanisms underlying the data-generating process, we demonstrate a way to detect unobserved confounders when having multiple observational datasets coming from different environments. We present a theory for testable conditional independencies that are only absent when there is hidden confounding and examine cases where we violate its assumptions: degenerate & dependent mechanisms, and faithfulness violations. Additionally, we propose a procedure to test these independencies and study its empirical finite-sample behavior using simulation studies and semi-synthetic data based on a real-world dataset. In most cases, the proposed procedure correctly predicts the presence of hidden confounding, particularly when the confounding bias is large.

==> tables/jci_table.tex <==
\begin{table}[]
\caption{Conditional d-separations in combinations of DAGs with variables $(T, Y, U)$. For the d-separation, (\cmark) indicates that it holds and (\xmark) otherwise. The gray shaded rows are the cases where $E\rightarrow U$, while yellow shaded is without an edge between $E$ and $U$. }
\label{tab:jci_table}
\centering
\begin{tabular}{rlllllll}
\toprule
id & \rot{$T - Y$} & \rot{$U - T$} & \rot{$U - Y$} & \rot{$E - T$} & \rot{$E - U$} & \rot{$U$ is confounder} & \rot{$Y \perp_d E \mid T$}\\
\midrule
\cellcolor{yellow}{1} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\cmark} & \cellcolor{yellow}{\xmark}\\
\cellcolor{lightgray}{2} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{3} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{4} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{5} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\addlinespace
\cellcolor{yellow}{6} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{7} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{8} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{9} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{10} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\addlinespace
\cellcolor{yellow}{11} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{12} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{13} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{14} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{15} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\addlinespace
\cellcolor{yellow}{16} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{17} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{18} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\cmark} & \cellcolor{yellow}{\xmark}\\
\cellcolor{lightgray}{19} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{20} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\addlinespace
\cellcolor{lightgray}{21} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{22} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{23} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{24} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{25} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\addlinespace
\cellcolor{yellow}{26} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{27} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{28} & \cellcolor{yellow}{} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{29} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{30} & \cellcolor{yellow}{} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\leftarrow$} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\addlinespace
\cellcolor{lightgray}{31} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\leftarrow$} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{lightgray}{32} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\cellcolor{yellow}{33} & \cellcolor{yellow}{} & \cellcolor{yellow}{} & \cellcolor{yellow}{} & \cellcolor{yellow}{$\rightarrow$} & \cellcolor{yellow}{} & \cellcolor{yellow}{\xmark} & \cellcolor{yellow}{\cmark}\\
\cellcolor{lightgray}{34} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{} & \cellcolor{lightgray}{$\rightarrow$} & \cellcolor{lightgray}{\xmark} & \cellcolor{lightgray}{\cmark}\\
\bottomrule
\end{tabular}
\end{table}

==> tikz/plate_v2.tex <==
\begin{tikzpicture}

    % variables
    \node[state] (t) at (0,0) {$T_i^{(k)}$};

    \node[state] (y) at (2,0) {$Y_i^{(k)}$};
    
    \node[state] (x) [above =of t ] {$X_i^{(k)}$};

    \node[latent] (u) [above =of y ] {$U_i^{(k)}$};
    
    % causal mechanisms
    \node[latent] (tX) [above =of x] {$\mX^{(k)}$};
    \node[latent] (tU) [above =of u] {$\mU^{(k)}$};
    \node[latent] (tT) [left=of tX] {$\mT^{(k)}$};
    \node[latent] (tY) [right=of tU] {$\mY^{(k)}$};
    
    % directed edges
    \path (t) edge (y);
    \path (u) edge (y);
    \path (u) edge (t);
    \path (x) edge (y);
    \path (x) edge (t);
    \path (x) edge (u);
    \path (tT) edge[bend right=30] (t);
    \path (tY) edge[bend left=30]  (y);
    \path (tU) edge (u);
    \path (tX) edge (x);
    
    % plate
    \plate [inner sep=.25cm,xshift=.02cm,yshift=.2cm] {plate1} {(t) (y) (x) (u)} {Samples $i=1,2,\dots,N_{k}$};
    \plate [inner sep=0.5cm,xshift=.02cm,yshift=-.2cm] {plate2} {(t) (y) (x) (u) (tX) (tU) (tT) (tY)} {Environments $k=1,2,\dots,K$};
    

\end{tikzpicture}
